Holistic-Motion2D: Scalable Whole-body Human Motion Generation in 2D Space

In this paper, we introduce a novel path to $\textit{general}$ human motion generation by focusing on 2D space. Traditional methods have primarily generated human motions in 3D, which, while detailed and realistic, are often limited by the scope of available 3D motion data in terms of both the size and the diversity. To address these limitations, we exploit extensive availability of 2D motion data. We present $\textbf{Holistic-Motion2D}$, the first comprehensive and large-scale benchmark for 2D whole-body motion generation, which includes over 1M in-the-wild motion sequences, each paired with high-quality whole-body/partial pose annotations and textual descriptions. Notably, Holistic-Motion2D is ten times larger than the previously largest 3D motion dataset. We also introduce a baseline method, featuring innovative $\textit{whole-body part-aware attention}$ and $\textit{confidence-aware modeling}$ techniques, tailored for 2D $\underline{\text T}$ext-driv$\underline{\text{EN}}$ whole-bo$\underline{\text D}$y motion gen$\underline{\text{ER}}$ation, namely $\textbf{Tender}$. Extensive experiments demonstrate the effectiveness of $\textbf{Holistic-Motion2D}$ and $\textbf{Tender}$ in generating expressive, diverse, and realistic human motions. We also highlight the utility of 2D motion for various downstream applications and its potential for lifting to 3D motion. The page link is: https://holistic-motion2d.github.io.

==> tables/datasets_comparison.tex <==
\begin{figure}[t]
    % \vspace{-3em}
    \begin{center}
        \centerline{\includegraphics[width=\linewidth]{figures/2D-3D.pdf}}
        \vspace{-2mm}
        \caption{Comparison of estimating 3D keypoints (SPIN \cite{kolotouros2019learning}) and direct prediction of 2D keypoints (RTMPose~\cite{jiang2023rtmpose}) from images. The precision of 2D keypoints demonstrates robustness to variations in viewpoint.}
        \label{fig:2D-3D}
    \end{center}
    % \vspace{-0.9cm}
\end{figure}

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{1.4mm}

\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{3}{c}{Motion Annotation} & \multicolumn{2}{c}{Text Annotation} & \multicolumn{2}{c}{Scene} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}RGB\\    Image\end{tabular}} \\ 
                         & Clip       & Holistic    & Hours    & Motion          & Holistic        & Indoor      & Outdoor     &                                                                         \\ \midrule
KIT-ML~\cite{plappert2016kit}                   & 3,911       & No            & 11.2     & 6,278            & No                & Yes         & No          & No                                                                      \\
AMASS~\cite{mahmood2019amass}                    & 11,265      & No            & 40.0     & 0               & No                & Yes         & No          & No                                                                      \\
BABEL~\cite{punnakkal2021babel}                    & 13,220      & No            & 43.5     & 91,408           & No                & Yes         & No          & No                                                                      \\
HumanAct12~\cite{guo2020action2motion}               & 1,191          & No            & 6.0        & 1,191               & No                & Yes         & No          & No                                                                      \\
HumanML3D~\cite{guo2022generating}                & 14,616      & No            & 28.6     & 44,970           & No                & Yes         & No          & No                                                                      \\
Motion-X~\cite{lin2024motion}                 & 95,642      & No           & 127.1    & 95,642           & Yes               & Yes         & Yes         & Yes                                                                     \\
Holistic-Motion2D (ours)                     &  1,002,463   & Yes           &      1,614.5   & 1,002,463         & Yes               & Yes         & Yes         & Yes                                                                     \\ \bottomrule
\end{tabular}
\captionsetup{skip=2pt}
\caption{Comparison between our proposed Holistic-Motion2D and existing text-motion datasets. The video quantity of our Holistic-Motion2D is \textbf{10$\times$} larger than the previously largest 3D motion dataset, \textit{i.e.}, Motion-X.}
\label{tab: compared to other dataset}
% \vspace{-0.7cm}
\end{table}


